Visualizing Information Bottleneck through Variational Inference

The Information Bottleneck theory provides a theoretical and computational framework for finding approximate minimum sufficient statistics. Analysis of the Stochastic Gradient Descent (SGD) training of a neural network on a toy problem has shown the existence of two phases, fitting and compression. In this work, we analyze the SGD training process of a Deep Neural Network on MNIST classification and confirm the existence of two phases of SGD training. We also propose a setup for estimating the mutual information for a Deep Neural Network through Variational Inference.

==> backup.tex <==

\subsection{Student Model}

The student model is a feedforward network that learns to extract some signal $Y$ from $X$. In case of MNIST $Y$ would be the digit that the image $X$ is supposed to represent. We split the student into two parts: an $Encoder_{C}$ which defines a mapping $p(z_c | x)$ from the input to a hidden state $z_c$ and a $Classifier_{C}$ which takes $z_c$ as input and outputs the label probabilities $p(y| z_c)$ for $Y$.

Our method requires that $p(z_c | x)$ be probabilistic, furthermore that it is differentiable wrt $z_c$ and $x$. An example would be if $p(z_c | x) = \mathcal{N}(z_c | \mu(x), \Sigma(x))$, where $\mu$ and $\Sigma$ are differentiable neural nets that compute the parameters of a Gaussian given the image $x$. Such an encoder can be trained using the Variational Information Bottleneck \citep{DBLP:journals/corr/AlemiFD016} method, which can be seen as a generalization of VAE to the supervised setting.

\textbf{TODO: Replace Equation with VIB equation.}
\begin{equation}
  \max \limits_{\theta} \sum \limits_{i=1}^{N} \log (f(y^{(i)}, x^{(i)}, \theta))
\end{equation}

where $f(X; \theta)$ is a neural network parameterized by $\theta$ with the last layer being a softmax layer which outputs a 10 dimensional vector containing the probability of the 10 labels for the input image.

The architecture of our network is \textbf{TODO(Abhishek)}. The network is trained using gradient descent.

Our goal is to estimate $I(X; Z_c)$ and $I(Z_c; Y)$, the location of the network on the information plane. In the following sections we show how to estimate these quantities for teacher-student pairs that satisfy our requirements. We wish to find a method that finds good solutions in a short amount of time, such that it is possible to estimate the quantities multiple times during training.

\subsection{Variational Inference}

Variational Autoencoders (VAE) \citep{kingma2013autovae} is a generative model which deals with models of distributions $P(X)$, defined over datapoints $X$ in some potentially high-dimensional space $\mathcal{X}$. $X$ for our setup would be MNIST digits. VAE is a latent variable model in which we are aiming to maximize the probability of each $X$ in the training set under the entire generative process according to:

\begin{equation}
  P(X) = \int P(X|z_v;\beta)P(z_v) dz_v
\end{equation}

In VAEs, the choice of output distribution is Gaussian, i.e. $P(X|z_v; \beta) = \mathcal{N}(X|f(z_v;\beta), \sigma^2 I)$, $z_v$ is our latent variable.

In VAE $f(z_v; \beta)$ is a multi-layer neural network. The key idea behind VAE is to attempt to sample values of $z_v$ that are likely to have produce $X$, and compute $P(X)$ just from those. This means that we need a new function $Q(z_v|X)$ which can take a value of $X$ and give us a distribution over $z_v$ values that are likely to produce $X$. This allows us to compute $E_{z_v \sim Q}P(X|z_v)$ relatively easily. Now we need to relate $E_{z_v \sim Q}P(X|z_v)$ and $P(X)$ which can be done using variational Bayesian methods. For exact derivation refer to section 2.1 of \citet{doersch2016tutorial}. The final relation that we get is:

\begin{equation}
  \log P(X) - \mathcal{D}[Q(z|X) || P(z|X)] = E_{z \sim Q} [\log P(X|z)] - \mathcal{D}[Q(z|X) || P(z)]
\end{equation}

In the above equation, left hand side has the quantity we want to maximize: $\log P(X)$. The right hand side is something we can optimize via stochastic gradient descent.

\textbf{TODO(Abhishek): This can probably move to the background section.}

\subsection{Information Plane}

To calculate the Information Plane of the feedforward neural network at $Z_c$ we would need to calculate $I(X; Z_c)$ and $I(Z_c; Y)$.

\begin{enumerate}
  \item $I(X; Z_c)$
Now let us look at the second part of equation: $\mathbb{E}_{z_c} \log p(z_c)$.


  \textbf{TODO(Abhishek)}: Add a note about $Q$.

  \item $I(Z_C; Y)$: Estimating mutual information with respect to the output $Y$ is easy. For MNIST, $Y$ has 10 possible values. We structured $Encoder_{C}$ so that each hidden state belongs to a gaussian distribution and a mean and variance is output for each hidden state. Using this information you can exhaustively compute the mutual information $I(Z_C; Y)$.
\end{enumerate}

\textbf{TODO(Abhishek)}

